Online Learning for Mixture of Multivariate Hawkes Processes

Online learning of Hawkes processes has received increasing attention in the last couple of years especially for modeling a network of actors. However, these works typically either model the rich interaction between the events or the latent cluster of the actors or the network structure between the actors. We propose to model the latent structure of the network of actors as well as their rich interaction across events for real-world settings of medical and financial applications. Experimental results on both synthetic and real-world data showcase the efficacy of our approach.

==> OMMHP Arxiv/Algorithm.tex <==
It is difficult to directly work with the log-likelihood $$\log \big(\sum_k \pi^k \mathrm{HP}^{\delta}(\vs|\bm \mu^k,\bm \theta^k) \big)$$ due to summation inside the logarithm. 
%
Instead, we work with the evidence lower bound (ELBO) defined as %\cn~
%
\begin{align}
    \mathrm{ELBO}(\bm \Theta)= \E_{q(\mZ)}[L^{\delta}(\bm \Theta,\mZ)]- \E_{q(\mZ)}[\log q(\mZ)]
\end{align}
%
for a properly chosen distribution $q(\mZ)$, where $L^{\delta}(\bm \Theta, \mZ)$ is the complete log-likelihood defined as %Here, 
%$L^{\delta}(\vs|k)\triangleq \log \mathrm{HP}^{\delta}(\vs|\bm \mu^k,\bm \theta^k) \big)$ is the conditional log-likelihood and
%
\begin{align}
    L^{\delta}(\bm \Theta, \mZ)\triangleq& \sum_{n=1}^N\sum_{k=1}^K z_{nk}\Big[ \log \pi^{k} + \log \mathrm{HP}^{\delta}(\vs_n|\bm \mu^k,\bm \theta^k) \big)\Big]\nonumber\\
    %
    %&=\sum_{n=1}^N\Big[ \log \pi^{k_n} +  \sum\limits_{\tau=1}^{T/\delta}\sum\limits_{p=1}^{P}\big[ {x_{\tau,p}} \log (\lambda^k_{n,p}(\tau\delta)\big) -\delta   \lambda^k_{n,p}(\tau\delta) \big] \Big]\nonumber\\
    %
    = & \sum\limits_{\tau=1}^{T/\delta}\sum_{n=1}^N \sum\limits_{p=1}^{P}\sum_{k=1}^K z_{nk}\big[ x^{\tau}_{n,p} \log (\lambda^k_{n,p}(\tau\delta)\big) -\delta   \lambda^k_{n,p}(\tau\delta) \big] + \sum_{n=1}^N \sum_{k=1}^K z_{nk} \log \pi^{k} \nonumber \\
    %
    =&  \sum\limits_{\tau=1}^{T/\delta} L_{\tau}^{\delta}(\bm \Theta, \mZ)  + \sum_{n=1}^N \sum_{k=1}^K z_{nk} \log \pi^{k} 
\end{align}
%
is the complete log-likelihood function. The additive nature of $L^{\delta}(\bm \Theta, \mZ)$ allows for adopting online algorithms to maximize the ELBO function. We assume that $q(\mZ)$ takes the simple form $q(\mZ)=\prod_{n=1}^N q(\vz_n)$ where $q(\vz_n)\sim \mathrm{multinom}(\bm\alpha_n)$ and $\vz_n\in [K]$. Therefore,
%
\begin{align}
    \mathrm{ELBO}(\bm \Theta)%&= \sum\limits_{\tau=1}^{T/\delta} \E_{q(\mZ)}L_{\tau}^{\delta}(\bm \Theta, \mZ)  + \sum_{n=1}^N \sum_{k=1}^K \alpha_{nk} \log \pi^{k}  - \sum_{n=1}^N \sum_{k=1}^K \alpha_{nk} \log \alpha_{nk}\nonumber\\
    %
    &= \sum\limits_{\tau=1}^{T/\delta} \E_{q(\mZ)}L_{\tau}^{\delta}(\bm \Theta)  + \sum_{n=1}^N \sum_{k=1}^K \alpha_{nk} \log \pi^{k}/\alpha_{nk} 
\end{align}
%
with
%
\begin{align*}
 \E_{q(\mZ)}L_{\tau}^{\delta}(\bm \Theta, \mZ)  =  \sum_{n=1}^N \sum\limits_{p=1}^{P} \sum_{k=1}^K \alpha_{nk} \big[ x^{\tau}_{n,p} \log (\lambda^k_{n,p}(\tau\delta)\big) -\delta   \lambda^k_{n,p}(\tau\delta) \big] .
 \end{align*}
%
This allows us to employ the online variational inference framework for mixture models employed by \cite{sato2001online}, \cite{hoffman2010online}, and \cite{fang2020online}. The $t$-th iteration of  OMMHP consists of the following two steps:

\paragraph{E-Step (responsibilities update):} Due to the independence assumption on cluster assignments ($q(\mZ)=\prod_{n=1}^N q(\vz_n)$), we can adopt a coordinate descent procedure for updating the responsibilities, i.e., we alternatingly maximize the ELBO function with respect to $\bm \alpha_n$:
%
\begin{align}
    \alpha_{nk}^t &\propto \pi^k(t-1) \underbrace{\exp\left(\sum_{\tau=1}^t\sum_{p=1}^P \big[ {x^{\tau}_{n,p}} \log (\lambda^k_{n,p}(\tau\delta)\big) -\delta   \lambda^k_{n,p}(\tau\delta) \big]\right)}_{R^{t}(k,n)}\nonumber%\\
    %
    %&\propto \pi^k(t-1)\cdot \exp\Big(\sum_{p=1}^P \big[ {x_{t,p}} \log (\lambda^k_{n,p}(t\delta)\big) -\delta \lambda^k_{n,p}(t\delta) \big]\Big)\cdot S^{t-1}(k,n)
\end{align}
%
where $$R^{t}(k,n) = \exp \left(\sum\nolimits_{p=1}^P \big[ x^{t}_{n,p} \log (\lambda^k_{n,p}(t\delta)\big) -\delta \lambda^k_{n,p}(t\delta) \big]\right)\cdot R^{t-1}(k,n)$$ can be computed recursively and $\pi^k(t-1)$ is the estimate of $\pi^k$ after observing the $(t-1)$-th interval (i.e. at the beginning of the $t$-th interval). It follows trivially that $\alpha_{nk}^t=\frac{\pi^k(t-1) R^{t}(k,n)}{\sum_{k=1}^K \pi^k(t-1) R^{t}(k,n)}$ and $\pi^k(t)=\sum_{n=1}^N \alpha_{nk}^t /N$.
 
 
 
\paragraph{M-Step (HP parameters update):} %\nic{Here we need to update the wording. Right now we are fitting the M-step as in the Morse's thesis \cite{morse2017persistent}, who in turns cites \cite{veen2008hawkesEM, Ke2013Hawkes, zipkin2016hawkes}. We could say something like ``we include the gradients in case one wants to use it, but for the experiments we use the M-step as in the papers above.''} 

The M-step of \textbf{OMMHP} framework involves updating parameters $\mu^k_p$ and $\theta^k_{p^i,p^j}$. This can be done by a variety of methods including expectation-minimization (EM) as proposed in \cite[Chapter 5]{morse2017persistent}, or using stochastic gradient updates. More details on the M-step can be found in Appendix B.  
The pseudo-code for \textbf{OMMHP} 
is presented in Algorithm \ref{algo:ommhp}. 

 \begin{algorithm}[t]
\caption{Online mixture of multivariate Hawkes Processes (\textbf{OMMHP})} \label{algo:ommhp}
\begin{algorithmic}[1]
\REQUIRE $K$, $P$, $T$, $\mS$ , $\delta$
%
\STATE Initialize $\{R^0(k,n)\}$,  $\{\bm\alpha_n(0)\}$, $\{\bm\mu^k(0)\}$, $\{\bm\theta^k(0)\}$
%
\FOR{$t=1$ to $T/\delta$}
%
\STATE Observe new events in $(\delta(t-1),\delta t]$ for all sequences
\STATE Set the step size $\eta_{t}$ 
%
%\FOR{$p=1$ to $p$}
%        \STATE calculate  $x^{t}_{n,p}$
%\ENDFOR
%
\STATE E-step:
\FOR{$n=1$ to $N$}
\FOR{$k=1$ to $K$}
\FOR{$p=1$ to $P$}
\STATE $\lambda^k_{n,p}(t\delta) = \mu^k_{p}(t-1) + \sum\limits_{i_n: t_{i_n}<t} f^k(t\delta-t_{i_n}; \theta_{p_{i_n} p}(t-1))$
\ENDFOR
\STATE $R^{t}(k,n) = \exp(\sum\limits_{p=1}^P \big[ x^{t}_{n,p} \log (\lambda^k_{n,p}(t\delta)\big) -\delta \lambda^k_{n,p}(t\delta) \big])\cdot R^{t-1}(k,n)$
%
\ENDFOR
\FOR{$k=1$ to $K$}
\STATE $\alpha_{nk}^t=\frac{\pi^k(t-1) R^{t}(k,n)}{\sum_{k=1}^K \pi^k(t-1) R^{t}(k,n)}$
\ENDFOR
\ENDFOR
\FOR{$k=1$ to $K$}
\STATE $\pi^k(t)=\sum_{n=1}^N \alpha_{nk}^t /N$
\ENDFOR
\STATE M-step: %EM or Stochastic Gradient %(Stochastic gradient approach):
\STATE Use estimation algorithm for $\mu_p^k$ and $\theta^k_{p^i, p^j}$, such as EM \cite{zipkin2016hawkes} or stochastic gradient descent (see Appendix~\ref{sec:sgd_updates})

%\mg{Apply EM or stochastic gradient approach}
%\FOR{$k=1$ to $K$}
%\STATE $\bm \mu^k(t) = \bm \mu^k(t-1) + \eta_{t} \frac{\partial \E_{q^{t-1}(\mZ)}L_{t}^{\delta}(\bm \Theta, \mZ)}{\partial \bm \mu^k }$ 
%,
%\STATE $\bm \theta^k(t) = \bm \theta^k(t-1) + \eta_{t} \frac{\partial \E_{q^{t-1}(\mZ)}L_{t}^{\delta}(\bm \Theta, \mZ)}{\partial \bm \theta^k }$ 
%\ENDFOR
%

%
%%\STATE $\pi^k(t)=\sum_{n=1}^N \alpha_{nk}^t /N$
%%\STATE Update $\lambda^k_{n,p}$ for $n\in [N]$, $p\in [P]$, and $K\in[K]$
%%\STATE $\lambda^k_p(t) = \mu^k_p + \sum_{i: t_i<t} f^k(t-t_i; \theta_{p_i p})$ for $n\in [N]$, $p\in [P]$, and $K\in[K]$
%%\RETURN 
\ENDFOR
\end{algorithmic}
\end{algorithm}



==> OMMHP Arxiv/Network_short.tex <==

%\section{Network formulation}
Consider an online stream of events of the form $s=\{e,t)\}$ with timestamp $t$ and event $e$. 
We assume that the event data corresponds to an interaction between two nodes on a network $A$. 
Mathematically, we can enumerate the set of events for a network as $\mathbf{E} = \{(i,j,p) \in A \times [P]\}$.
We model these event sequences using a mixture of Hawkes processes. Specifically, for type $p$ event sequences between nodes $i$ and $j$ the intensity function at time $t$ is given by:
%
\begin{align}\label{mixture-network}
\lambda_{i,j,p}(t) = \mu_{z_i,z_j,p} + \sum_{l: t_l<t} f_{z_i,z_j}(t-t_l; \theta_{p_l,p})   
\end{align}
where $\mu_{z_i,z_j,p}$ is the base intensity for the event type $p$ corresponding to the nodes $i,j$ and $z_i \in [K], z_j \in [K]$ denote their cluster memberships. %Following similar steps as in Sections \ref{sec:prob_def} and \ref{sec:algo} , the ELBO function obtains the following form:
Notice that in the scenario where the nodes do not interact with each other and events correspond only to the individual node, the problem can be reduced to our setting as follows. It is a special case of our formulation by considering a bipartite network with the same set of nodes on each side with links mapping to the different event types between the corresponding duplicate nodes.

 




\subsection{ELBO}
The log-likelihood of our sequence when the labels of the nodes are known is given by 
$$\log \big(\sum_{k_1,k_2} \pi_{k_1,k_2} \mathrm{HP}^{\delta}(\vs|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2}) \big).$$ due to summation inside the logarithm. 
%
Instead, we work with the evidence lower bound (ELBO) defined as %\cn~
%
\begin{align}
    \mathrm{ELBO}(\bm \Theta)= \E_{q(\bm z)}[L^{\delta}(\bm \Theta,\bm z)]- \E_{q(\bm z)}[\log q(\bm z)]
\end{align}
%
for a properly chosen distribution $q(\bm z)$, where $L^{\delta}(\bm \Theta, \bm z)$ is the complete log-likelihood defined as %Here, 
%$L^{\delta}(\vs|k)\triangleq \log \mathrm{HP}^{\delta}(\vs|\bm \mu^k,\bm \theta^k) \big)$ is the conditional log-likelihood and
%
\begin{align}
    &L^{\delta}(\bm \Theta, \mZ) \triangleq \sum_{(i,j) \in A}\sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2}\Big[ \log \mathrm{HP}^{\delta}(\vs_{i,j}|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2}) + \log \pi_{k_1,k_2} \Big]\nonumber\\
    %
    %&=\sum_{n=1}^N\Big[ \log \pi^{k_n} +  \sum\limits_{\tau=1}^{T/\delta}\sum\limits_{p=1}^{P}\big[ {x_{\tau,p}} \log (\lambda^k_{n,p}(\tau\delta)\big) -\delta   \lambda^k_{n,p}(\tau\delta) \big] \Big]\nonumber\\
    %
    &=  \sum\limits_{\tau=1}^{T/\delta}\sum_{(i,j) \in A} \sum\limits_{p=1}^{P}\sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2}\big[ x^{\tau}_{i,j,p} \log (\lambda_{i,j,k_1,k_2,p}(\tau\delta)\big)  \big] \nonumber\\
    &\quad -\sum\limits_{\tau=1}^{T/\delta}\sum_{(i,j) \in A} \sum\limits_{p=1}^{P}\sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2}\big[ \delta   \lambda_{i,j,k_1,k_2,p}(\tau\delta) \big]  + \sum_{(i,j) \in A} \sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2} \log \pi_{k_1,k_2}  \nonumber\\
    %
    &=  \sum\limits_{\tau=1}^{T/\delta} L_{\tau}^{\delta}(\bm \Theta, \bm z)  + \sum_{(i,j) \in A} \sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2} \log \pi_{k_1,k_2} 
\end{align}
%
is the complete log-likelihood function.
The additive nature of $L_{\tau}^{\delta}(\bm \Theta, \bm z)$ allows for adopting online algorithms to maximize the ELBO function. We assume that $q(\bm z)$ takes the simple form $q(\bm z)=\prod_{n=1}^N q(\vz_n)$ where $q(\vz_n)\sim \mathrm{multinom}(\bm\alpha_n)$ and $\vz_n\in [K]$. Therefore,
%
\begin{align}
    \mathrm{ELBO}(\bm \Theta)&= \sum\limits_{\tau=1}^{T/\delta} \E_{q(\bm z)}L_{\tau}^{\delta}(\bm \Theta, \bm z)  + \sum_{n=1}^N \sum_{k_1=1}^K\sum_{k_2=1}^K \alpha_{i,k_1}\alpha_{j,k_2} \log \pi_{k_1,k_2}  \nonumber\\
    &\qquad- \sum_{(i,j)\in A} \sum_{k_1=1}^K\sum_{k_2=1}^K\alpha_{i,k_1}\alpha_{j,k_2} \log \alpha_{i,k_1}\alpha_{j,k_2}%\nonumber\\
    %
    %&= \sum\limits_{\tau=1}^{T/\delta} \E_{q(\mZ)}L_{\tau}^{\delta}(\bm \Theta)  + \sum_{n=1}^N \sum_{k=1}^K \alpha_{nk} \log \pi^{k}/\alpha_{nk} 
\end{align}
%
with
%
\begin{align}
 &\E_{q(\bm z)}L_{\tau}^{\delta}(\bm \Theta, \bm z)  = \sum_{(i,j)\in A} \sum\limits_{p=1}^{P} \sum_{k_1=1}^K\sum_{k_2=1}^K \alpha_{i,k_1} \alpha_{j,k_2}\big[ x^{\tau}_{i,j,p} \log (\lambda_{k_1,k_2,p}(\tau\delta)\big)  \big] \nonumber\\
 %
&\qquad\qquad-\sum_{(i,j)\in A} \sum\limits_{p=1}^{P} \sum_{k_1=1}^K\sum_{k_2=1}^K \alpha_{i,k_1} \alpha_{j,k_2}\big[ \delta   \lambda_{k_1,k_2,p}(\tau\delta) \big] .
 \end{align}
%
The OMMHP can be applied here in a similar fashion to Section \ref{sec:algo}. %We omit details due to lack of space.
%This allows us to employ the online variational inference framework for mixture models employed by \cite{sato2001online}, \cite{hoffman2010online}, and \cite{fang2020online}. The $t$-th iteration of the our online algorithm OMMHP consists of the following two steps:


==> OMMHP Arxiv/experiments.tex <==
\section{Experiments}  %\nic{02/18: Draft ready, feel free to change the language as much as you'd like.}
We validate the effectiveness of \textbf{OMMHP} in learning the underlying parameters of a mixture of Hawkes processes on both synthetic and real-world data.



\subsection{Synthetic Data} \label{sec:synth_data}
We generate two sets of synthetic datasets mixing the following Hawkes processes:

\begin{align*}
    \mathbf{x} &\sim HP\left(\bm \mu_1 = [0.3, 0.2], \bm a_1 =
\begin{bmatrix}
     0.2 & 0.1 \\ 0.1 & 0.2
\end{bmatrix} \right) \\
\mathbf{y} &\sim HP\left(\bm \mu_2 = [2.8, 1.6], \bm a_2 = 
\begin{bmatrix}0.6 & 0.2 \\ 0.2 & 0.6
\end{bmatrix} \right) \\
\mathbf{z} &\sim HP\left(\bm \mu_3 = [1.4, 0.8], \bm a_3 =
\begin{bmatrix}
     0.4 & 0.0 \\ 0.0 & 0.6
\end{bmatrix} \right)
\end{align*}

In the first dataset we generate $n=10$ sequences from the first two processes, so $\mathcal{D}_1 = \left \{ (\mathbf{x_i})_{i=1}^{n}, (\mathbf{y_j})_{j=1}^{n}  \right \}$, while in the second dataset we generate $n=10$ sequences from all processes, so $\mathcal{D}_2 = \left \{ (\mathbf{x_i})_{i=1}^{n}, (\mathbf{y_j})_{j=1}^{n}, (\mathbf{z_k})_{k=1}^{n}  \right \}$. In both datasets we set $T=1000$ and the decay rate to $u = 3.1$.

We apply \textbf{OMMHP}  on both these dataset to recover the mixture identities of the sequences and learn the parameters of the Hawkes processes. 
We chose $\delta=25$ and update the parameters using a $\eta_t=\frac{1}{\sqrt{t+1}}$ decay, a standard decay rate commonly used in online learning literature \cite{hall2016tracking}. In both cases the correct cluster assignments is learned by \textbf{OMMHP}. Moreover, Figure~\ref{fig:convergence} shows the convergence of the learned parameters to the true parameters as a function of the iteration. We compute the relative difference in $\ell_2$ norm for vectors and Frobenius norms for matrices for the learned and true parameter values. As baseline, we provide the relative error in estimating each cluster parameters using accelerated gradient descent (using the \texttt{tick} package by \cite{bacry2017tick}, shown in dashed lines in Figure~\ref{fig:convergence}). \textbf{OMMHP} achieves relative errors which are comparable to off-the-shelf algorithms that have access to the true cluster labels. In addition, we investigate the convergence behavior as a function of the number of generated sequences $n$ for each process. Figure~\ref{fig:convergence_function_realization_2HP} shows that for the mixture of two Hawkes processes the parameter convergence is generally faster if a higher number of sequences from each process is observed, which is the expected behavior. However, a higher number of sequences $n$ improves the estimation error more significantly for the first process in the mixture, which indicates the first process is the hardest to estimate among the two. A similar takeaway applies to the mixture of three Hawkes processes case, which we include in Figure~\ref{fig:convergence_function_realization_3HP} in Appendix~\ref{appendixc: experiments}. Finally, we also include an empirical study showing the estimation process scales roughly linearly in the number of generated sequences $n$, event types, and mixture components; see Figure~\ref{fig:scaling_plot_ommhp} and Table~\ref{tab:scaling} in Appendix~\ref{appendixc: experiments} for details.


\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.53\linewidth]{figures/synthetic_2clusters.pdf}  
    \hspace{-1cm}
    \includegraphics[width=0.53\linewidth]{figures/synthetic_3clusters.pdf}
    \caption{Convergence plot for the mixtures of 2 (left) and 3 (right) Hawkes processes with $n=10$ observed sequences. OMMHP relative errors are reported computing the $\ell_2$ norms (for baselines $\mu_i$) and Frobenius norms (for adjacency matrices $\bm a_i$) in solid lines. Dashed lines indicate the relative error achieved by accelerated gradient descent when using true cluster labels. OMMHP correctly recovers the correct cluster assignment and achieves relative errors which are comparable to off-the-shelf algorithms that have access to the true cluster labels. For details see Section~\ref{sec:synth_data}.}
    \label{fig:convergence}
\end{figure*}


\begin{figure*}[!h]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/parameter_convergence_2mixture_function_of_realization.pdf}  
    \caption{Convergence plot for the mixtures of 2 Hawkes processes as a function of the generated number of sequences $n$. OMMHP relative errors are reported computing the $\ell_2$ norms (for baselines $\mu_i$) and Frobenius norms (for adjacency matrices $\bm a_i$) in solid lines. As expected, a higher number of generated sequences $n$ leads to a faster convergence, although with different behaviors between the two processes in the mixture. For details see Section~\ref{sec:synth_data}.}
    \label{fig:convergence_function_realization_2HP}
\end{figure*}



\subsection{Real Data} \label{sec:real_data}

To showcase \textbf{OMMHP}'s performance on real-world data we consider two real-world datasets: (1) the \textit{MathOverflow} dataset \cite{leskovec2014snap}, which tracks the interaction between users on a question-answering forum between the years of 2009 and 2016 and (2) the \textit{MOOC} dataset \cite{feng2019dropout}, which tracks the actions of students of a massive online open course held virtually by a Chinese university. Throughout this section we use the adjusted Rand index (ARI, \cite{rand1971objective}) as clustering performance metric. If the clustering performance is roughly equivalent to random clustering, the ARI will be equal to zero, while a better-than-chance performance is reflected by a positive ARI. For both experiments we fit OMMHP using Algorithm~\ref{algo:ommhp} with $\eta_t=\frac{1}{\sqrt{t+1}}$.


\subsubsection{MathOverflow Dataset}

This dataset is structured so that each interaction is recorded as a pair of users (sender and receiver) and a timestamp for when the interaction occurred. As there are no details on the interaction type, we grouped all interactions together as a single even type. We select the interactions coming from the 100 most active users, selected as the union of the set of the 50 most active senders and 50 users who have received the most interactions in the dataset, for a total of $\sim 170,000$ interactions. We first compute a series of activity-related features, such as the total years of activity, total interactions and average monthly interactions, project such features using the Isomap algorithm \cite{tenenbaum2000global}\footnote{We found that clustering in the original feature space did not lead to any meaningful clustering behavior.} and cluster the users using the \texttt{k-means++} clustering algorithm. We select $6$ as the final number of clusters using the elbow method \cite{marutho2018determination,bock2008inertiakmeans}.%, that is, the sum of the square distances sharply increases when adding more clusters 
(see Figure~\ref{fig:elbow_plots}, left, in Appendix~\ref{appendixc: experiments}). The results is three large cluster (more than 20 users), one medium clusters (with 12) and a series of small size cluster (with less than 8 users each). OMMHP clustering achieves a better-than-chance final ARI of 0.1 on such clustering. To demonstrate the robustness of our approach, Figure\ref{fig:mathoverflow_clustering_performance} shows that OMMHP achieves better-than-chance clustering performance across various number of clusters (between 2 and 10) and projection algorithms (original data space, Isomap, t-SNE \cite{vandermaaten2008tsne} and locally linear embedding \cite{saul2000introduction}). 


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/mathoverflow_clustering_performance.pdf}  
    \caption{Clustering performance (indicated by ARI) across various clusters and projection methods for the MathOverflow dataset. %Using OMMHP for detecting clusters results in a better-than-chance clustering performance, indicated by a consistently positive ARI. 
    For details see Section~\ref{sec:real_data}.}
    \label{fig:mathoverflow_clustering_performance}
\end{figure}


\begin{table*}[!h]
%\vspace{-0.4\baselineskip}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\multicolumn{10}{c}{\textit{MOOC Clustering Performance}} \\
\hline
 & \multicolumn{9}{|c|}{\textbf{Clusters}} \\
 \hline
 & 2 & 3 & \textbf{\textcolor{red}{4}} & 5 & 6 & 7 & 8 & 9 & 10 \\
\hline
\textbf{Adjusted Rand Index} & -0.047 & 0.025 & \textbf{\textcolor{red}{0.201}}  & 0.150 & 0.00 & 0.129& 0.107& 0.064& 0.098 \\
\hline
\end{tabular}
\vspace{0.5\baselineskip}
\caption{Clustering performance (indicated by ARI) across various cluster numbers for the MOOC dataset. Using OMMHP for detecting clusters mostly results in a better-than-chance clustering performance, indicated by an ARI larger than zero. The performance for the number of clusters chosen via the ``elbow method''is highlighted in red. For details see Section~\ref{sec:real_data}.} \label{tab:mooc_performance}
\end{table*}

\subsubsection{MOOC Dataset}

The MOOC dataset tracks the behavior of around $150,000$ students enrolled in 250 online open courses held by a Chinese university. All student actions, such as play a video, stop a video or click on a problem, are recorded in the dataset along with the timestamp of the action. In order to reduce the dimensionality of the dataset, we first select the most common 9 actions and group all other actions into the same category, hence creating 10 event types. Some students in the dataset perform almost the same action thousand of times, we filter such students. We then select the top 25 students across all courses, leaving a total of $\sim 365,000$ actions. Similarly to what performed above, we cluster the students based on the actions performed during their experience with the online class using the \texttt{k-means++} clustering algorithm; we select $4$ as the final number of clusters, since the inertia stops decreasing significantly when using more clusters (Figure~\ref{fig:elbow_plots}, right, for the inertia plot). The four clusters are composed of three balanced clusters with 8 students each, and cluster with a single student, for which using OMMHP for clustering achieves a better-than-chance ARI of $0.2$. Similarly for what shown above for the MathOverflow dataset, Table~\ref{tab:mooc_performance} reports the ARI for different cluster numbers, showing how using OMMHP for clustering usually achieves better-than-chance clustering results. 










==> OMMHP Arxiv/macros.tex <==
%packages

\usepackage{mathtools}
\usepackage{amssymb,latexsym,amsmath, mathtools,bm,amsthm}
\usepackage{color}
\usepackage[dvipsnames]{xcolor}
\usepackage{amssymb}
\usepackage{bbm,mathrsfs}
%\usepackage[keeplastbox]{flushend}
%\usepackage{csquotes}
%\usepackage{subcaption}
%\usepackage{enumitem}
\usepackage{multicol,multirow}
%\usepackage[normalem]{ulem}
\usepackage{setspace}
%----------------------------------------------------------------------------------------
%NEW COMMANDS
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{sketchofproof}{Sketch of proof}
\newtheorem{remark}{Remark}

%----------------------------------------------------------------------------------------
% Define some commands to keep the formatting separated from the content 


%% typefaces
\def\mb{\mathbb}
\def\mbf{\mathbf}
\def\mc{\mathcal}
\def\mk{\mathfrak}
\def\ms{\mathscr}
\def\m{\mathbf}

%% functions and operators
%\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\ip}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\br}[1]{\left[#1 \right]}
\newcommand{\pr}[1]{\left(#1 \right)}
\newcommand{\nor}[1]{\left\|#1 \right\|}
\newcommand{\tr}{\mathop{\mathrm{Tr}}\nolimits}
\newcommand{\supp}{\mathop{\mathrm{supp}}\nolimits}
\newcommand{\vect}{\mathop{\mathrm{vec}}\nolimits}
\newcommand{\diag}{\mathop{\mathrm{diag}}\nolimits}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\E}{\mb{E}}
\renewcommand{\P}{\mb{P}}
\newcommand{\soft}{\mathop{\mathrm{softmax}}\nolimits}
\def\Diag{\mathop{\mathrm{Diag}}}
%\def\diag{\mathop{\mathrm{diag}}}

%% special notation


\newcommand{\nul}{\mathop{\mathrm{Null}}\nolimits}
\newcommand{\col}{\mathop{\mathrm{Col}}\nolimits}
\newcommand{\row}{\mathop{\mathrm{Row}}\nolimits}

\newcommand{\h}[1]{\hat{\mbf{#1}}}
\newcommand{\wt}[1]{\widetilde{\mbf{#1}}}
\newcommand{\ldel}{\underline\delta}
\renewcommand{\v}[1]{\mbf{#1}}
\renewcommand{\m}[1]{\v{#1}}

% todos
%\usepackage[colorinlistoftodos,color=orange!70,textsize=scriptsize,shadow]{todonotes}
%\newcommand{\note}[1]{\namedtodo{NOTE}{#1}{color=red!40}}
\newcommand{\stodo}[2][]{\todo[caption={#2},#1]{\begin{spacing}{0.8}#2\end{spacing}}}
\newcommand{\namedtodo}[3]{\todo[caption={#2},#3]{\begin{spacing}{0.8}\textbf{\uppercase{#1}:} {#2}\end{spacing}}}
\newcommand{\todo}[1]{\textcolor{ForestGreen}{\textbf{TODO:} #1}}
\newcommand\redout{\bgroup\markoverwith{\textcolor{red}{\rule[.5ex]{2pt}{0.4pt}}}\ULon}
\newcommand{\edit}[2]{\redout{#1}{~\textcolor{blue}{#2}}}
\newcommand{\cn}{\textcolor{red}{[\raisebox{-0.2ex}{\tiny\shortstack{citation\\[-1ex]needed}}]}~}
\newcommand{\mg}[1]{\textcolor{blue}{\textbf{MG:} #1}}
\newcommand{\nd}[1]{\textcolor{brown}{\textbf{ND:} #1}}
\newcommand{\ek}[1]{\textcolor{red}{\textbf{EK:} #1}}
\newcommand{\vp}[1]{\textcolor{brown}{\textbf{VP:} #1}}



\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

==> OMMHP Arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{algorithmic,algorithm}
\usepackage{mathtools}
\usepackage{latexsym,amsmath, mathtools}
\usepackage{color}
\usepackage{bbm,mathrsfs}

\usepackage{pifont}







% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


%\setlength{\marginparwidth}{2cm}
% \usepackage[backgroundcolor=white]{todonotes}
% \newcommand{\stodo}[2][]{\todo[caption={#2},#1]{\begin{spacing}{0.8}#2\end{spacing}}}
% \newcommand{\namedtodo}[3]{\todo[caption={#2},#3]{\begin{spacing}{0.8}\textbf{\uppercase{#1}:} {#2}\end{spacing}}}
% %\newcommand{\todo}[1]{\textcolor{Green}{\textbf{TODO:} #1}}
% \newcommand{\mg}[1]{\textcolor{blue}{\textbf{MG:} #1}}
% \newcommand{\nic}[1]{\textcolor{red}{\textbf{ND:} #1}}
% \newcommand{\todov}[2][]{\todo[color=green!20,size=\tiny,inline,#1]{V: #2}} % Vamsi's comments
% \newcommand\redout{\bgroup\markoverwith{\textcolor{red}{\rule[.5ex]{2pt}{0.4pt}}}\ULon}
% \newcommand{\edit}[2]{\redout{#1}{~\textcolor{blue}{#2}}}
% \newcommand{\cn}{\textcolor{red}{[\raisebox{-0.2ex}{\tiny\shortstack{citation\\[-1ex]needed}}]}}

%% extra symbol

% \newcommand{\cmark}{\ding{51}}%
% \newcommand{\xmark}{\ding{55}}%

==> OMMHP Arxiv/network.tex <==

%\section{Network formulation}
Consider an online stream of events of the form $s=\{e,t)\}$ with timestamp $t$ and event $e$. 
We assume that the event data corresponds to an interaction between two nodes on a network $A$. 
Mathematically, we can enumerate the set of events for a network as $\mathbf{E} = \{(i,j,p) \in A \times [P]\}$.
We model these event sequences using a mixture of Hawkes processes. Specifically, for type $p$ event sequences between nodes $i$ and $j$ the intensity function at time $t$ is given by:
%
\begin{align}\label{mixture-network}
\lambda_{i,j,p}(t) = \mu_{z_i,z_j,p} + \sum_{l: t_l<t} f_{z_i,z_j}(t-t_l; \theta_{p_l,p})   
\end{align}
where $\mu_{z_i,z_j,p}$ is the base intensity for the event type $p$ corresponding to the nodes $i,j$ and $z_i \in [K], z_j \in [K]$ denote their cluster memberships. 
 In this work, we assume the impact functions are exponentials in the form of $f_{z_i, z_j}(t-t_l; \theta_{p_l ,p})  = a_{z_i,z_j,p_l, p} \exp\big(-b_{z_i,z_j,p_i, p} (t-t_l)\big)$
where $\theta_{z_i,z_j,p_i,p}=(a_{z_i,z_j,p_i,p}, b_{z_i,z_j,p_i,p})$. Define $\bm \theta_{k_1,k_2}=(\theta_{k_1,k_2,p_i,p_j}) _{p_i\in[P], p_j\in[P]}$ and $\bm \mu_{k_1,k_2}= (\mu_{k_1,k_2,p})_{p\in[P]}$, and $\bm \Theta=(\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2})_{k_1\in[K],k_2\in[K]}$.
 Then, the probability of observing a sequence $\vs$ (in time interval [0,T]) can be described as 
%
\begin{align}
    P(\vs;\bm \Theta) = \sum_{k_1=1}^K\sum_{k_2=1}^{K} \pi_{k_1,k_2}~ \mathrm{HP} (\vs|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2})
\end{align}
where 
\begin{align*}
&\mathrm{HP} (\vs|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2})=\nonumber\\ &\qquad\qquad\prod\limits_{i: t_i<T} \lambda_{k_1,k_2,p_i}(t_i) \exp\Big(-\sum_{p=1}^P\int_{0}^T \lambda_{k_1,k_2,p}(s) ds\Big)
\end{align*}
and $\{\pi_{k_1,k_2}\}$ are the probabilities of the clusters.

Notice that in the scenario where the nodes do not interact with each other and events correspond only to the individual node, the problem can be reduced to our setting as follows. It is a special case of our formulation by considering a bipartite network with the same set of nodes on each side with links mapping to the different event types between the corresponding duplicate nodes.

 
\paragraph{Discretized Loss Function}

We discretize the point process by partitioning time into intervals of length $\delta$ and evaluate the likelihood functions at the end of the intervals. Let us denote $N_{p,t}$ by the number of events between nodes up to time $t$.  Let $x_{\tau,p}=N_{p, \tau\delta}-N_{p, (\tau-1)\delta}$ be the number of events of type $p$ that occurred during the $\tau^{\mathrm{th}}$ time interval. We can then discretize the conditional likelihood function $\mathrm{HP}^{\delta} (\vs|\bm \mu^k,\bm \theta^k)$ as 
%
\begin{align}
    %L^{\delta}(\bm\Theta|z=k) \triangleq 
    &\mathrm{HP}^{\delta} (\vs|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2})\nonumber\\
    &\quad\qquad= \prod\limits_{\tau=1}^{T/\delta}\prod\limits_{p=1}^{P} \Big[ (\lambda_{k_1,k_2,p}(\tau\delta)\big)^{x_{\tau,p}} \exp\big(- \delta   \lambda_{k_1,k_2,p}(\tau\delta)) \Big]
\end{align}
%
Consequently, the discretized likelihood function can be written as 
%
%
\begin{align}
    %L^{\delta}(\bm\Theta) \triangleq 
    &P^{\delta}(\vs;\bm \Theta)= \nonumber\\
    & \sum_{k_1=1}^K \sum_{k_2=1}^K \pi_{k_1,k_2}~ \prod\limits_{\tau=1}^{T/\delta}\prod\limits_{p=1}^{P}\Big[ (\lambda_{k_1,k_2,p}(\tau\delta)\big)^{x_{\tau,p}} \exp\big(- \delta   \lambda_{k_1,k_2,p}(\tau\delta)) \Big]\nonumber
\end{align}

%\subsection{ELBO}
%The log-likelihood of our sequence when the labels of the nodes are known is given by:
%\begin{align}
%    l(\bm \Theta| \textbf{z}) &= \sum_{(i,j)\in A} \sum_{p} \int_{0}^{T} \log \lambda_{i,j,p}(t|z) dN_{i,j}(t) - \sum_{p{'}}\int_{0}^{T} \lambda_{i,j,p{'}}(t|z) dt
%\end{align}
%We have the complete log-likelihood as follows:
%\begin{align*}
%    l(\bm \Theta, \textbf{z}) = \sum_{i=1}^m \log \pi_{z_i} + l(\bm \Theta|\textbf{z})
%\end{align*}
%We can write out the ELBO as follows:
%\begin{align}
%    \mathrm{ELBO}(\bm \Theta) = \E_{q(\textbf{Z})} l(\bm \Theta, \textbf{z}) - \E_{q(\textbf{Z})} \log q(\textbf{z})
%\end{align}
%The final form is given by:
%\begin{align}
%    \mathrm{ELBO} = \sum_{n=1}^{N} \E_{q(\bm Z)} l_n(\bm \Theta| \bm z) +   \sum_i \sum_k \tau_{ik} \log \pi_k/\tau_{ik}
%\end{align}
%where $q(\bm Z) = \prod_i q_i(z_i)$, $q_i(z) = \textrm{multinom}(\tau_i)$ with $\tau_i \in \mathcal{R}^k$ and the bucketed term is given by:
%\begin{align}
%    \E_{q(\bm Z)} l_n(\bm \Theta, \bm z) &= \sum_{(i,j)\in A, p_l}  \int_{(n-1)dT}^{ndT} \log \lambda_{i,j,p_l}(t|z) dN_{i,j}(t) - \sum_{p}\int_{(n-1)dT}^{ndT} \lambda_{i,j,p}(t|z) dt
%\end{align}
\subsection{Online Learning of Hawkes Processes}
It is difficult to directly work with the log-likelihood $$\log \big(\sum_{k_1,k_2} \pi_{k_1,k_2} \mathrm{HP}^{\delta}(\vs|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2}) \big)$$ due to summation inside the logarithm. 
%
Instead, we work with the evidence lower bound (ELBO) defined as %\cn~
%
\begin{align}
    \mathrm{ELBO}(\bm \Theta)= \E_{q(\bm z)}[L^{\delta}(\bm \Theta,\bm z)]- \E_{q(\bm z)}[\log q(\bm z)]
\end{align}
%
for a properly chosen distribution $q(\bm z)$, where $L^{\delta}(\bm \Theta, \bm z)$ is the complete log-likelihood defined as %Here, 
%$L^{\delta}(\vs|k)\triangleq \log \mathrm{HP}^{\delta}(\vs|\bm \mu^k,\bm \theta^k) \big)$ is the conditional log-likelihood and
%
\begin{align}
    &L^{\delta}(\bm \Theta, \mZ)\nonumber\\
    &\triangleq \sum_{(i,j) \in A}\sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2}\Big[ \log \mathrm{HP}^{\delta}(\vs_{i,j}|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2}) + \log \pi_{k_1,k_2} \Big]\nonumber\\
    %
    %&=\sum_{n=1}^N\Big[ \log \pi^{k_n} +  \sum\limits_{\tau=1}^{T/\delta}\sum\limits_{p=1}^{P}\big[ {x_{\tau,p}} \log (\lambda^k_{n,p}(\tau\delta)\big) -\delta   \lambda^k_{n,p}(\tau\delta) \big] \Big]\nonumber\\
    %
    &=  \sum\limits_{\tau=1}^{T/\delta}\sum_{(i,j) \in A} \sum\limits_{p=1}^{P}\sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2}\big[ x^{\tau}_{i,j,p} \log (\lambda_{i,j,k_1,k_2,p}(\tau\delta)\big)  \big] \nonumber\\
    &\quad -\sum\limits_{\tau=1}^{T/\delta}\sum_{(i,j) \in A} \sum\limits_{p=1}^{P}\sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2}\big[ \delta   \lambda_{i,j,k_1,k_2,p}(\tau\delta) \big]\nonumber \\
    &\quad + \sum_{(i,j) \in A} \sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2} \log \pi_{k_1,k_2}  \nonumber\\
    %
    &=  \sum\limits_{\tau=1}^{T/\delta} L_{\tau}^{\delta}(\bm \Theta, \bm z)  + \sum_{(i,j) \in A} \sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2} \log \pi_{k_1,k_2} 
\end{align}
%
is the complete log-likelihood function. The additive nature of $L^{\delta}(\bm \Theta, \bm z)$ allows for adopting online algorithms to maximize the ELBO function. We assume that $q(\bm z)$ takes the simple form $q(\bm z)=\prod_{n=1}^N q(\vz_n)$ where $q(\vz_n)\sim \mathrm{multinom}(\bm\alpha_n)$ and $\vz_n\in [K]$. Therefore,
%
\begin{align}
    \mathrm{ELBO}(\bm \Theta)&= \sum\limits_{\tau=1}^{T/\delta} \E_{q(\bm z)}L_{\tau}^{\delta}(\bm \Theta, \bm z)  + \sum_{n=1}^N \sum_{k_1=1}^K\sum_{k_2=1}^K \alpha_{i,k_1}\alpha_{j,k_2} \log \pi_{k_1,k_2}  \nonumber\\
    &\qquad- \sum_{(i,j)\in A} \sum_{k_1=1}^K\sum_{k_2=1}^K\alpha_{i,k_1}\alpha_{j,k_2} \log \alpha_{i,k_1}\alpha_{j,k_2}%\nonumber\\
    %
    %&= \sum\limits_{\tau=1}^{T/\delta} \E_{q(\mZ)}L_{\tau}^{\delta}(\bm \Theta)  + \sum_{n=1}^N \sum_{k=1}^K \alpha_{nk} \log \pi^{k}/\alpha_{nk} 
\end{align}
%
with
%
\begin{align}
 &\E_{q(\bm z)}L_{\tau}^{\delta}(\bm \Theta, \bm z)  = \nonumber\\
 %
 &\sum_{(i,j)\in A} \sum\limits_{p=1}^{P} \sum_{k_1=1}^K\sum_{k_2=1}^K \alpha_{i,k_1} \alpha_{j,k_2}\big[ x^{\tau}_{i,j,p} \log (\lambda_{k_1,k_2,p}(\tau\delta)\big)  \big] \nonumber\\
 %
 &\qquad\qquad-\sum_{(i,j)\in A} \sum\limits_{p=1}^{P} \sum_{k_1=1}^K\sum_{k_2=1}^K \alpha_{i,k_1} \alpha_{j,k_2}\big[ \delta   \lambda_{k_1,k_2,p}(\tau\delta) \big] .
 \end{align}
%
This allows us to employ the online variational inference framework for mixture models employed by \cite{sato2001online}, \cite{hoffman2010online}, and \cite{fang2020online}. The $t$-th iteration of the our online algorithm OMMHP consists of the following two steps:

\paragraph{E-Step (responsibilities update):} Due to the independence assumption on cluster assignments ($q(\bm z)=\prod_{i=1}^N q(\vz_i)$), we can adopt a coordinate descent procedure for updating the responsibilities, i.e., we alternatingly maximize the ELBO function with respect to $\bm \alpha_n$:
%
\begin{align}
    &\alpha_{i,k_1}^t \propto \pi_{k_1}(t-1)\cdot\nonumber\\
    %
    &\underbrace{\exp\Big(\sum_{\tau=1}^t\sum_{j: (i,j) \in A}\sum_{p=1}^P \big[ {x^{\tau}_{i,j,p}} \log (\lambda_{i,j,k_1,k_2,p}(\tau\delta)\big) -\delta   \lambda_{i,j,k_1,k_2,p}(\tau\delta) \big]\Big)}_{R^{t}(k_1,i)}%\nonumber\\
    %
    %&\propto \pi^k(t-1)\cdot \exp\Big(\sum_{p=1}^P \big[ {x_{t,p}} \log (\lambda^k_{n,p}(t\delta)\big) -\delta \lambda^k_{n,p}(t\delta) \big]\Big)\cdot S^{t-1}(k,n)
\end{align}
%
where $R^{t}(k_1,i) = \exp(\sum_{j: (i,j) \in A}\sum_{p=1}^P \big[ x^{\tau}_{i,j,p} \log (\lambda_{i,j,k_1,k_2,p}(\tau\delta)\big) -\delta \lambda_{i,j,k_1,k_2,p}(\tau\delta) \big])\cdot R^{t-1}(k_1,i)$ can be computed recursively and $\pi_{k_1}(t-1)$ is the estimate of $\pi_{k_1}$ after observing the $(t-1)$-th interval (i.e. at the beginning of the $t$-th interval). It follows trivially that $\alpha_{n,k}^t=\frac{\pi^k(t-1) R^{t}(k,n)}{\sum_{k=1}^K \pi^k(t-1) R^{t}(k,n)}$ and $\pi_k(t)=\sum_{n=1}^N \alpha_{n,k}^t /N$.
 
 
 
\paragraph{M-Step (HP parameters update):} In the M-step of OMMHP, we perform a (stochastic) gradient update on the parameters of the Hawkes processes. This is in contrast to the batch model where the objective is alternatingly minimized w.r.t. each parameter of the Hawkes processes.  
\begin{align*}
     &\mu_{k_1,k_2,p}(t) =  \mu_{k_1,k_2,p}({t-1}) + \eta_{t} \frac{\partial \E_{q^{t-1}(\bm z)}L_{t}^{\delta}(\bm \Theta, \bm z)}{\partial  \mu_{k_1,k_2,p} }\\  &\theta_{k_1,k_2,p^i,p^j}(t) =  \theta_{k_1,k_2,p_i,p_j}(t-1) + \eta_{t} \frac{\partial \E_{q^{t-1}(\mZ)}L_{t}^{\delta}(\bm \Theta, \bm z)}{\partial  \theta_{k_1,k_2,p_i,p_j} }
\end{align*}
%\mg{I think it would be interesting if we took into account the impact of different edges of the same node on each other. This would allow for clustering of the events. In the format of this section (with $z_i$ and $z_j$'s), it is not possible to do that: right now different event types are on the same edge. Consider the example of journeys data.  Under current model, all customers are connected to ONE node on the other side, and one each edge we can have different event types. Since we have only one node (the bank), on the other side, there is no clustering to be done. Another option would be to consider each event as a node. Since we have around 2000 events, we need a bipartite graph where on one side we have customers and on the other side we have 2000 nodes representing the events. In this case $P=1$, since we put the events on the nodes, so it doesn't make sense to say there are different event types on each edge. In this case, finding different event types is equivalent to clustering the event nodes (this reduces to the setup of 2020 paper). However neither in the 2020 paper nor in the model proposed in this section (with $z_i$ and $z_j$'s), the impact of different events on each other is not taken into account. }


%\mg{ Now, if we allow for event on different edges to impact each other, we can cluster the event based on how they impact each other. This would be the most general case that would subsume all possible types of interactions. I think this is a very interesting use-case and can differentiate our work even more from the 2020 paper.}

%\mg{For the algorithm we can just keep what we have though. We can say we develop an algorithm for a special case of our model which is the same as 2017 paper. We can talk about other spacial cases in the appendix. After all, they allow even position paper that only propose ideas.}

%\todov{I am not sure I follow the stuff about customer journeys. So, to do customer journeys in the current model you would take n nodes and create a bipartite network with 2n nodes with each node connected to its clone. Yup, we can make the model more complex --- consider a node and let all its events be considered across all its neighbors and edge types when building the intensity function. However, if we do that I think that should be a full paper.}

%\todov{Also if you allow a nodes events to influence each other, you lose the link-level modeling that we are proposing here. So, its not super-set to what we have here. Could be interesting to explore modeling in this space but it is out of scope for this paper.}

==> intro.tex <==
In many applications we need to deal with large number of sequences of events that occur asynchronously and at irregular intervals. Examples of such sequential data include interactions of customers with a bank (customers journeys), customers purchases at a grocery/online store, visits of patients to a hospital, and spread of viral diseases such as COVID-19~\cite{yan2019recent, mei2017neural,zuo2020transformer,browning2021simple, garetto2021time}. Each event sequence can consist of multiple events of different types. %\mg{Consider interactions of customers with a bank (known in banking nomenclatures as customers journeys). Some of these interactions can be prompted by earlier interactions and may require to be attended by a specialist. }
Predicting the time and the type of the next event for each sequence, finding the possible latent cluster of actors~\cite{xu2017dirchlet}, inferring causal relations between events~\cite{xu2016causality}, and deliberately influencing the behaviors of the actors~\cite{farajtabar2014shaping}~are some interesting applications when dealing with sequential data.


Due to irregular and asynchronous nature of sequential events data, the standard time-series approaches are not able to capture the rich information that exist in occurrence times of such data. Instead, point processes are commonly used to learn the distribution of sequential event data. Specifically, multivariate Hawkes processes (MHP) have received considerable attention in the recent years due to their ability to model triggering (or inhibiting) effect of past events of different type on future events~\cite{rasmussen2018lecture}. Many works in the literature focus on employing non-parametric as well as neural network based approaches to design impact functions that are able to model complex dependencies of events in point processes~\cite{mei2017neural,zuo2020transformer,zhang2019self}. Despite the outstanding results, a limitation of the aforementioned works is that they learn a single dependency pattern for all the sequences of events. To address this shortcoming, \cite{xu2017dirchlet} propose a \textit{mixture of multivariate Hawkes processes} (MMHP) which  allow for modeling event
sequences where there exist multiple impact
patterns across the
sequences. The mixture model allows for identifying latent clustering structures across event sequences. 

In this work, we propose \textit{online learning for mixture of multivariate Hawkes processes} (\textbf{OMMHP}). The online learning framework addresses scalability issues of batch models by reducing the per iteration computational complexity. Moreover, in many applications such as banking, shopping, and health care we deal with streaming sequences of events. It is often the case that the behaviors of the actors, i.e. the dependencies between events, change over time, possibly abruptly. Similarly, the cluster structures can change over time, with people moving from one cluster to another (e.g. due to a change in employment status) or with new clusters emerging and old clusters disappearing. The drastic changes that many communities are going through due to the recent COVID-19 pandemic emphasizes the dynamic nature of the underlying models of sequential data in many applications \cite{garetto2021time,chiang2020hawkes}. Online learning of MMHP allows to identify and model this dynamic nature without the need for the costly process of training models from scratch. To the best of our knowledge, this paper presents the first online MMHP framework that takes into account the interactions and dependencies between different types of events.




%Learning these distributions allow for predicting the time and type of the next event in each sequence.


%\todov{plate model}


 \subsection{Related Work}
 
 %Mei and Eisner \cite{mei2017neural} proposed using continuous time LSTMs to model the conditional intensity function in point processes to address the limitations of earlier works in modeling complex dependencies of events in point processes. Recently, inspired by the success of attention mechanism in natural language processing \cn, computer vision\cn, and many other areas, Zuo et al \cite{Zuo2020transformer} and Zhang et al. \cite{zhang2019self} proposed using transformers instead of LSTM networks.
 

\paragraph{Clustering of Point Processes}
While many of the existing work on clustering point processes focus on clustering subsequences of events within the sequences in order to find common patterns \cite{Du2015dirichlet,turkmen2020clustering}, some recent art have addressed the challenging problem of clustering the sequences themselves. Most notably, \cite{xu2017dirchlet} propose a probabilistic mixture model that aims at modeling sequences that are generated from a mixture of self-triggering Hawkes processes. Along similar lines, \cite{sharma2019generative} propose a generative model that allows for modeling mixtures of more complex point processes through the use of recurrent models such as RNNs and LSTMs.
 
 \paragraph{Online Learning of Point Processes}
 
\cite{hall2016tracking} propose a parametric online framework for learning Hawkes processes. In contrast, \cite{yang2017online} propose a non-parametric approach that allows for more complex interaction functions. Most recently, \cite{fang2020online} proposed an online community detection algorithm based on sequences of interactions among nodes in a network. We propose a general model which encompasses the setting in \cite{fang2020online} by considering the multivariate case where we allow for multiple event types (types of interaction) to occur between the nodes.
\begin{table}[t!]
\caption{Prior art on online learning of point processes}
%\vspace{-0.4\baselineskip}
\label{table:network}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Paper & sequence clustering & event interactions & network \\
\hline
\cite{hall2016tracking} & \xmark  &  \xmark & \cmark\\
\hline
\cite{yang2017online} & \xmark  &  \cmark  & \xmark\\
\hline
\cite{fang2020online} & \cmark  &  \xmark  & \cmark\\
\hline
This work & \cmark  &  \cmark  & \cmark\\
\hline
\end{tabular}
%\vspace{-0.2\baselineskip}
\end{table}
Table~\ref{table:network} contains a comparison of our model versus the existing models in the literature. For ease of exposition, we present an online framework for learning the mixture of Hawkes processes with event interactions and defer the full version of incorporating the network structure to the appendix.  
%\todov{Table is optimistic, need to add the network component: currently it looks like we subsume all the remaining models: we don't}





%\begin{table*}[t]
%\caption{Prior art on online learning of point processes}
%\vspace{-0.4\baselineskip}
%\label{table:bib}
%\centering
%\begin{tabular}{|c|c|c|}
%\hline
%Paper & sequence clustering & event interactions  \\
%\hline
%\cite{hall2016tracking} & \xmark  &  \xmark \\
%\hline
%\cite{yang2017online} & \xmark  &  \cmark  \\
%\hline
%\cite{fang2020online} & \cmark  &  \xmark  \\
%\hline
%This work & \cmark  &  \cmark  \\
%\hline
%\end{tabular}
%\vspace{-0.2\baselineskip}
%\end{table*}


==> network.tex <==

%\section{Network formulation}
Consider an online stream of events of the form $s=\{e,t)\}$ with timestamp $t$ and event $e$. 
We assume that the event data corresponds to an interaction between two nodes on a network $A$. 
Mathematically, we can enumerate the set of events for a network as $\mathbf{E} = \{(i,j,p) \in A \times [P]\}$.
We model these event sequences using a mixture of Hawkes processes. Specifically, for type $p$ event sequences between nodes $i$ and $j$ the intensity function at time $t$ is given by:
%
\begin{align}\label{mixture-network}
\lambda_{i,j,p}(t) = \mu_{z_i,z_j,p} + \sum_{l: t_l<t} f_{z_i,z_j}(t-t_l; \theta_{p_l,p})   
\end{align}
where $\mu_{z_i,z_j,p}$ is the base intensity for the event type $p$ corresponding to the nodes $i,j$ and $z_i \in [K], z_j \in [K]$ denote their cluster memberships. 
 In this work, we assume the impact functions are exponentials in the form of $f_{z_i, z_j}(t-t_l; \theta_{p_l ,p})  = a_{z_i,z_j,p_l, p} \exp\big(-b_{z_i,z_j,p_i, p} (t-t_l)\big)$
where $\theta_{z_i,z_j,p_i,p}=(a_{z_i,z_j,p_i,p}, b_{z_i,z_j,p_i,p})$. Define $\bm \theta_{k_1,k_2}=(\theta_{k_1,k_2,p_i,p_j}) _{p_i\in[P], p_j\in[P]}$ and $\bm \mu_{k_1,k_2}= (\mu_{k_1,k_2,p})_{p\in[P]}$, and $\bm \Theta=(\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2})_{k_1\in[K],k_2\in[K]}$.
 Then, the probability of observing a sequence $\vs$ (in time interval [0,T]) can be described as 
%
\begin{align}
    P(\vs;\bm \Theta) = \sum_{k_1=1}^K\sum_{k_2=1}^{K} \pi_{k_1,k_2}~ \mathrm{HP} (\vs|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2})
\end{align}
where 
\begin{align*}
&\mathrm{HP} (\vs|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2})=\nonumber\\ &\qquad\qquad\prod\limits_{i: t_i<T} \lambda_{k_1,k_2,p_i}(t_i) \exp\Big(-\sum_{p=1}^P\int_{0}^T \lambda_{k_1,k_2,p}(s) ds\Big)
\end{align*}
and $\{\pi_{k_1,k_2}\}$ are the probabilities of the clusters.

Notice that in the scenario where the nodes do not interact with each other and events correspond only to the individual node, the problem can be reduced to our setting as follows. It is a special case of our formulation by considering a bipartite network with the same set of nodes on each side with links mapping to the different event types between the corresponding duplicate nodes.

 
\paragraph{Discretized Loss Function}

We discretize the point process by partitioning time into intervals of length $\delta$ and evaluate the likelihood functions at the end of the intervals. Let us denote $N_{p,t}$ by the number of events between nodes up to time $t$.  Let $x_{\tau,p}=N_{p, \tau\delta}-N_{p, (\tau-1)\delta}$ be the number of events of type $p$ that occurred during the $\tau^{\mathrm{th}}$ time interval. We can then discretize the conditional likelihood function $\mathrm{HP}^{\delta} (\vs|\bm \mu^k,\bm \theta^k)$ as 
%
\begin{align}
    %L^{\delta}(\bm\Theta|z=k) \triangleq 
    &\mathrm{HP}^{\delta} (\vs|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2})\nonumber\\
    &\quad\qquad= \prod\limits_{\tau=1}^{T/\delta}\prod\limits_{p=1}^{P} \Big[ (\lambda_{k_1,k_2,p}(\tau\delta)\big)^{x_{\tau,p}} \exp\big(- \delta   \lambda_{k_1,k_2,p}(\tau\delta)) \Big]
\end{align}
%
Consequently, the discretized likelihood function can be written as 
%
%
\begin{align}
    %L^{\delta}(\bm\Theta) \triangleq 
    &P^{\delta}(\vs;\bm \Theta)= \nonumber\\
    & \sum_{k_1=1}^K \sum_{k_2=1}^K \pi_{k_1,k_2}~ \prod\limits_{\tau=1}^{T/\delta}\prod\limits_{p=1}^{P}\Big[ (\lambda_{k_1,k_2,p}(\tau\delta)\big)^{x_{\tau,p}} \exp\big(- \delta   \lambda_{k_1,k_2,p}(\tau\delta)) \Big]\nonumber
\end{align}

%\subsection{ELBO}
%The log-likelihood of our sequence when the labels of the nodes are known is given by:
%\begin{align}
%    l(\bm \Theta| \textbf{z}) &= \sum_{(i,j)\in A} \sum_{p} \int_{0}^{T} \log \lambda_{i,j,p}(t|z) dN_{i,j}(t) - \sum_{p{'}}\int_{0}^{T} \lambda_{i,j,p{'}}(t|z) dt
%\end{align}
%We have the complete log-likelihood as follows:
%\begin{align*}
%    l(\bm \Theta, \textbf{z}) = \sum_{i=1}^m \log \pi_{z_i} + l(\bm \Theta|\textbf{z})
%\end{align*}
%We can write out the ELBO as follows:
%\begin{align}
%    \mathrm{ELBO}(\bm \Theta) = \E_{q(\textbf{Z})} l(\bm \Theta, \textbf{z}) - \E_{q(\textbf{Z})} \log q(\textbf{z})
%\end{align}
%The final form is given by:
%\begin{align}
%    \mathrm{ELBO} = \sum_{n=1}^{N} \E_{q(\bm Z)} l_n(\bm \Theta| \bm z) +   \sum_i \sum_k \tau_{ik} \log \pi_k/\tau_{ik}
%\end{align}
%where $q(\bm Z) = \prod_i q_i(z_i)$, $q_i(z) = \textrm{multinom}(\tau_i)$ with $\tau_i \in \mathcal{R}^k$ and the bucketed term is given by:
%\begin{align}
%    \E_{q(\bm Z)} l_n(\bm \Theta, \bm z) &= \sum_{(i,j)\in A, p_l}  \int_{(n-1)dT}^{ndT} \log \lambda_{i,j,p_l}(t|z) dN_{i,j}(t) - \sum_{p}\int_{(n-1)dT}^{ndT} \lambda_{i,j,p}(t|z) dt
%\end{align}
\subsection{Online Learning of Hawkes Processes}
It is difficult to directly work with the log-likelihood $$\log \big(\sum_{k_1,k_2} \pi_{k_1,k_2} \mathrm{HP}^{\delta}(\vs|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2}) \big)$$ due to summation inside the logarithm. 
%
Instead, we work with the evidence lower bound (ELBO) defined as %\cn~
%
\begin{align}
    \mathrm{ELBO}(\bm \Theta)= \E_{q(\bm z)}[L^{\delta}(\bm \Theta,\bm z)]- \E_{q(\bm z)}[\log q(\bm z)]
\end{align}
%
for a properly chosen distribution $q(\bm z)$, where $L^{\delta}(\bm \Theta, \bm z)$ is the complete log-likelihood defined as %Here, 
%$L^{\delta}(\vs|k)\triangleq \log \mathrm{HP}^{\delta}(\vs|\bm \mu^k,\bm \theta^k) \big)$ is the conditional log-likelihood and
%
\begin{align}
    &L^{\delta}(\bm \Theta, \mZ)\nonumber\\
    &\triangleq \sum_{(i,j) \in A}\sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2}\Big[ \log \mathrm{HP}^{\delta}(\vs_{i,j}|\bm \mu_{k_1,k_2},\bm \theta_{k_1,k_2}) + \log \pi_{k_1,k_2} \Big]\nonumber\\
    %
    %&=\sum_{n=1}^N\Big[ \log \pi^{k_n} +  \sum\limits_{\tau=1}^{T/\delta}\sum\limits_{p=1}^{P}\big[ {x_{\tau,p}} \log (\lambda^k_{n,p}(\tau\delta)\big) -\delta   \lambda^k_{n,p}(\tau\delta) \big] \Big]\nonumber\\
    %
    &=  \sum\limits_{\tau=1}^{T/\delta}\sum_{(i,j) \in A} \sum\limits_{p=1}^{P}\sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2}\big[ x^{\tau}_{i,j,p} \log (\lambda_{i,j,k_1,k_2,p}(\tau\delta)\big)  \big] \nonumber\\
    &\quad -\sum\limits_{\tau=1}^{T/\delta}\sum_{(i,j) \in A} \sum\limits_{p=1}^{P}\sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2}\big[ \delta   \lambda_{i,j,k_1,k_2,p}(\tau\delta) \big]\nonumber \\
    &\quad + \sum_{(i,j) \in A} \sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2} \log \pi_{k_1,k_2}  \nonumber\\
    %
    &=  \sum\limits_{\tau=1}^{T/\delta} L_{\tau}^{\delta}(\bm \Theta, \bm z)  + \sum_{(i,j) \in A} \sum_{k_1=1}^K\sum_{k_2=1}^K z_{i,j,k_1,k_2} \log \pi_{k_1,k_2} 
\end{align}
%
is the complete log-likelihood function. The additive nature of $L^{\delta}(\bm \Theta, \bm z)$ allows for adopting online algorithms to maximize the ELBO function. We assume that $q(\bm z)$ takes the simple form $q(\bm z)=\prod_{n=1}^N q(\vz_n)$ where $q(\vz_n)\sim \mathrm{multinom}(\bm\alpha_n)$ and $\vz_n\in [K]$. Therefore,
%
\begin{align}
    \mathrm{ELBO}(\bm \Theta)&= \sum\limits_{\tau=1}^{T/\delta} \E_{q(\bm z)}L_{\tau}^{\delta}(\bm \Theta, \bm z)  + \sum_{n=1}^N \sum_{k_1=1}^K\sum_{k_2=1}^K \alpha_{i,k_1}\alpha_{j,k_2} \log \pi_{k_1,k_2}  \nonumber\\
    &\qquad- \sum_{(i,j)\in A} \sum_{k_1=1}^K\sum_{k_2=1}^K\alpha_{i,k_1}\alpha_{j,k_2} \log \alpha_{i,k_1}\alpha_{j,k_2}%\nonumber\\
    %
    %&= \sum\limits_{\tau=1}^{T/\delta} \E_{q(\mZ)}L_{\tau}^{\delta}(\bm \Theta)  + \sum_{n=1}^N \sum_{k=1}^K \alpha_{nk} \log \pi^{k}/\alpha_{nk} 
\end{align}
%
with
%
\begin{align}
 &\E_{q(\bm z)}L_{\tau}^{\delta}(\bm \Theta, \bm z)  = \nonumber\\
 %
 &\sum_{(i,j)\in A} \sum\limits_{p=1}^{P} \sum_{k_1=1}^K\sum_{k_2=1}^K \alpha_{i,k_1} \alpha_{j,k_2}\big[ x^{\tau}_{i,j,p} \log (\lambda_{k_1,k_2,p}(\tau\delta)\big)  \big] \nonumber\\
 %
 &\qquad\qquad-\sum_{(i,j)\in A} \sum\limits_{p=1}^{P} \sum_{k_1=1}^K\sum_{k_2=1}^K \alpha_{i,k_1} \alpha_{j,k_2}\big[ \delta   \lambda_{k_1,k_2,p}(\tau\delta) \big] .
 \end{align}
%
This allows us to employ the online variational inference framework for mixture models employed by \cite{sato2001online}, \cite{hoffman2010online}, and \cite{fang2020online}. The $t$-th iteration of the our online algorithm OMMHP consists of the following two steps:

\paragraph{E-Step (responsibilities update):} Due to the independence assumption on cluster assignments ($q(\bm z)=\prod_{i=1}^N q(\vz_i)$), we can adopt a coordinate descent procedure for updating the responsibilities, i.e., we alternatingly maximize the ELBO function with respect to $\bm \alpha_n$:
%
\begin{align}
    &\alpha_{i,k_1}^t \propto \pi_{k_1}(t-1)\cdot\nonumber\\
    %
    &\underbrace{\exp\Big(\sum_{\tau=1}^t\sum_{j: (i,j) \in A}\sum_{p=1}^P \big[ {x^{\tau}_{i,j,p}} \log (\lambda_{i,j,k_1,k_2,p}(\tau\delta)\big) -\delta   \lambda_{i,j,k_1,k_2,p}(\tau\delta) \big]\Big)}_{R^{t}(k_1,i)}%\nonumber\\
    %
    %&\propto \pi^k(t-1)\cdot \exp\Big(\sum_{p=1}^P \big[ {x_{t,p}} \log (\lambda^k_{n,p}(t\delta)\big) -\delta \lambda^k_{n,p}(t\delta) \big]\Big)\cdot S^{t-1}(k,n)
\end{align}
%
where $R^{t}(k_1,i) = \exp(\sum_{j: (i,j) \in A}\sum_{p=1}^P \big[ x^{\tau}_{i,j,p} \log (\lambda_{i,j,k_1,k_2,p}(\tau\delta)\big) -\delta \lambda_{i,j,k_1,k_2,p}(\tau\delta) \big])\cdot R^{t-1}(k_1,i)$ can be computed recursively and $\pi_{k_1}(t-1)$ is the estimate of $\pi_{k_1}$ after observing the $(t-1)$-th interval (i.e. at the beginning of the $t$-th interval). It follows trivially that $\alpha_{n,k}^t=\frac{\pi^k(t-1) R^{t}(k,n)}{\sum_{k=1}^K \pi^k(t-1) R^{t}(k,n)}$ and $\pi_k(t)=\sum_{n=1}^N \alpha_{n,k}^t /N$.
 
 
 
\paragraph{M-Step (HP parameters update):} In the M-step of OMMHP, we perform a (stochastic) gradient update on the parameters of the Hawkes processes. This is in contrast to the batch model where the objective is alternatingly minimized w.r.t. each parameter of the Hawkes processes.  
\begin{align*}
     &\mu_{k_1,k_2,p}(t) =  \mu_{k_1,k_2,p}({t-1}) + \eta_{t} \frac{\partial \E_{q^{t-1}(\bm z)}L_{t}^{\delta}(\bm \Theta, \bm z)}{\partial  \mu_{k_1,k_2,p} }\\  &\theta_{k_1,k_2,p^i,p^j}(t) =  \theta_{k_1,k_2,p_i,p_j}(t-1) + \eta_{t} \frac{\partial \E_{q^{t-1}(\mZ)}L_{t}^{\delta}(\bm \Theta, \bm z)}{\partial  \theta_{k_1,k_2,p_i,p_j} }
\end{align*}
%\mg{I think it would be interesting if we took into account the impact of different edges of the same node on each other. This would allow for clustering of the events. In the format of this section (with $z_i$ and $z_j$'s), it is not possible to do that: right now different event types are on the same edge. Consider the example of journeys data.  Under current model, all customers are connected to ONE node on the other side, and one each edge we can have different event types. Since we have only one node (the bank), on the other side, there is no clustering to be done. Another option would be to consider each event as a node. Since we have around 2000 events, we need a bipartite graph where on one side we have customers and on the other side we have 2000 nodes representing the events. In this case $P=1$, since we put the events on the nodes, so it doesn't make sense to say there are different event types on each edge. In this case, finding different event types is equivalent to clustering the event nodes (this reduces to the setup of 2020 paper). However neither in the 2020 paper nor in the model proposed in this section (with $z_i$ and $z_j$'s), the impact of different events on each other is not taken into account. }


%\mg{ Now, if we allow for event on different edges to impact each other, we can cluster the event based on how they impact each other. This would be the most general case that would subsume all possible types of interactions. I think this is a very interesting use-case and can differentiate our work even more from the 2020 paper.}

%\mg{For the algorithm we can just keep what we have though. We can say we develop an algorithm for a special case of our model which is the same as 2017 paper. We can talk about other spacial cases in the appendix. After all, they allow even position paper that only propose ideas.}

%\todov{I am not sure I follow the stuff about customer journeys. So, to do customer journeys in the current model you would take n nodes and create a bipartite network with 2n nodes with each node connected to its clone. Yup, we can make the model more complex --- consider a node and let all its events be considered across all its neighbors and edge types when building the intensity function. However, if we do that I think that should be a full paper.}

%\todov{Also if you allow a nodes events to influence each other, you lose the link-level modeling that we are proposing here. So, its not super-set to what we have here. Could be interesting to explore modeling in this space but it is out of scope for this paper.}
